Metric Compatible Training for Online Backfilling in Large-Scale Retrieval

Backfilling is the process of re-extracting all gallery embeddings from upgraded models in image retrieval systems. It inevitably requires a prohibitively large amount of computational cost and even entails the downtime of the service. Although backward-compatible learning sidesteps this challenge by tackling query-side representations, this leads to suboptimal solutions in principle because gallery embeddings cannot benefit from model upgrades. We address this dilemma by introducing an online backfilling algorithm, which enables us to achieve a progressive performance improvement during the backfilling process while not sacrificing the final performance of new model after the completion of backfilling. To this end, we first propose a simple distance rank merge technique for online backfilling. Then, we incorporate a reverse transformation module for more effective and efficient merging, which is further enhanced by adopting a metric-compatible contrastive learning approach. These two components help to make the distances of old and new models compatible, resulting in desirable merge results during backfilling with no extra computational overhead. Extensive experiments show the effectiveness of our framework on four standard benchmarks in various settings.

==> sections/Method_metric_learning.tex <==
% !TEX root = ./../main.tex

\section{Distance Calibration}
\label{sec:metric_learning}

%\subsection{Motivation}
While the proposed rank merge technique with the basic reverse transformation module works well, there exists room for improvement in calibrating feature embedding spaces of both systems.
This section discusses the issues in details and presents how we figure them out.

\subsection{Cross-Model Contrastive Learning}
The objective in \eqref{eq:rev_basic} cares about the positive pairs  $\phi^\text{old}$ and $\phi^\text{rev}$ with no consideration of negative pairs, which can sometimes lead to misranked position.
To handle this issue, we employ a supervised contrastive learning loss~\cite{InfoNCE, khosla2020supervised} to consider both positive and negative pairs as follows:
%
\vspace{-0.1cm}
\begin{align}
\mathcal{L}_\text{CL} (\mathbf{x}_i, y_i) &= - \log \frac{\sum_{y_k=y_i} s_{ik}^\text{old}}{\sum_{y_k=y_i} s_{ik}^\text{old} + \sum_{y_k \neq y_i} s_{ik}^\text{old}},
\label{eq:cl}
\end{align}
where $s_{ij}^\text{old} = \exp\left(-\text{dist}\left(\phi^\text{rev}(\mathbf{x}_i), \phi^\text{old}(\mathbf{x}_j)\right) \right)$ and $y_i$ denotes the class membership of the $i^\text{th}$ sample.
For more robust contrastive training, we perform hard example mining for both the positive and negative pairs\footnote{For each anchor, we select the half of the examples in each of positive and negative labels based on the distances from the anchor.}.
Such a contrastive learning approach facilitates distance calibration and improves feature discrimination because it promotes separation of the positive and negative examples.




\begin{figure}
	\begin{center}
        \includegraphics[width=0.99\linewidth]{figures/cmcl.png}
        \vspace{-0.5cm}
	\end{center}
	\caption{Illustration of cross-model contrastive learning loss with backward retrieval system $\{ \phi^\text{old}, \phi^\text{rev} \}$ and new retrieval system $\{ \phi^\text{new}, \phi^\text{new} \}$.
	Two boxes with dotted lines corresponds to two terms in~\eqref{eq:cmcl}.
	For each retrieval system, the distances between positive pairs are learned to be both smaller than those of negative pairs in the two retrieval systems.
	}
	\label{fig:mccl}
	\vspace{-1mm}    
\end{figure}

Now, although the distances within the backward retrieval system $\{ \phi^\text{rev}, \phi^\text{old} \}$ become more comparable, they are still not properly calibrated in terms of the distances in the new retrieval system $\{ \phi^\text{new}, \phi^\text{new} \}$.
Considering distances in both retrieval systems jointly when we train the reverse transformation module, we can obtain more comparable distances and consequently achieve more reliable rank merge results.
From this perspective, we propose a cross-model contrastive learning loss as
%
\begin{align}
\label{eq:cmcl}
\mathcal{L}_\text{CMCL}&(\mathbf{x}_i, y_i) =  \\
&- \log \frac{\sum_{y_k=y_i} s^\text{old}_{ik} }{\sum_{y_k=y_i} s^\text{old}_{ik} + \sum_{y_k \neq y_i} s^\text{old}_{ik} + \sum_{y_k\neq y_i} s^\text{new}_{ik}  } \nonumber \\
&-\log \frac{\sum_{y_k=y_i} s^\text{new}_{ik} }{\sum_{y_k=y_i} s^\text{new}_{ik} + \sum_{y_k\neq y_i} s^\text{new}_{ik} + \sum_{y_k\neq y_i} s^\text{old}_{ik}  }, \nonumber 
\end{align}
where $s^\text{new}_{ij} = \exp(-\text{dist}\big(\phi^\text{new}(\mathbf{x}_i), \phi^\text{new}(\mathbf{x}_j)\big))$ and $s^\text{old}_{ij} = \exp(-\text{dist}\big(\phi^\text{rev}(\mathbf{x}_i), \phi^\text{old}(\mathbf{x}_j)\big))$.
Figure~\ref{fig:mccl} illustrates the concept of the loss function.
The positive pairs from the backward retrieval system $\{ \phi^\text{rev}, \phi^\text{old} \}$ are trained to locate closer to the anchor than not only the negative pairs from the same system but also the ones from the new system $\{ \phi^\text{new}, \phi^\text{new} \}$, and vice versa.
We finally replace \eqref{eq:rev_basic} with \eqref{eq:cmcl} for training the reverse transformation module.
Compared to~\eqref{eq:cl}, additional heterogeneous negative terms in the denominator of \eqref{eq:cmcl} play a role as a regularizer to make the distances from one model directly comparable to those from other one, which is desirable for our rank merge strategy.
\suseo{This loss term is somewhat similar to~\cite{ract}.
However, while \cite{ract} directly aims at feature compatibility with old space, our method focuses only on metric compatibility between two spaces for rank merge, because our merge framework does not require old and new models to be compatible to each other.
While achieving feature compatibility clearly sacrifice the discriminability of new model by being constrained to old model, our metric compatibility does not constrain the feature space by itself and allows more flexibility, resulting in superior merge results.
}

\subsection{Learnable New Feature Embedding}
Until now, we do not jointly train the reverse transformation module $\psi(\cdot)$ and the new feature extraction module $\phi^\text{new}(\cdot)$ as illustrated in  Figure~\ref{fig:rtm}.
This hampers the compatibility between the backward and new retrieval systems because the backward retrieval system $\{ \phi^\text{rev}, \phi^\text{old} \}$ is the only part to be optimized while the new system $\{ \phi^\text{new}, \phi^\text{new} \}$ is fixed.
To provide more flexibility, we add another transformation module $\rho(\cdot)$ on top of the new model as shown in Figure~\ref{fig:rtm_trainable}, where  $\rho^\text{new} = \rho(\phi^\text{new})$ and $\rho^\text{rev} = \psi(\rho(\phi^\text{new}))$.
In this setting, we use $\rho^\text{new}$ as the final new model instead of $\phi^\text{new}$, and our rank merge process employs $\{ \rho^\text{rev}, \phi^\text{old} \}$ and $\{ \rho^\text{new}, \rho^\text{new} \}$ eventually.
This strategy helps to achieve a better compatibility by allowing both systems to be trainable.

The final loss function to train the reverse transformation module has the identical form to $\mathcal{L}_\text{CMCL}$ in \eqref{eq:cmcl} except for the definitions of $s^\text{new}_{ij}$ and $s^\text{old}_{ij}$, which are given by
%
\begin{align}
s^\text{new}_{ij} &= \exp\left(-\text{dist}\left(\rho^\text{new}(\mathbf{x}_i), \rho^\text{new}(\mathbf{x}_j)\right)\right)  \\ 
s^\text{old}_{ij} &= \exp\left(-\text{dist}\left(\rho^\text{rev}(\mathbf{x}_i), \phi^\text{old}(\mathbf{x}_j)\right)\right). 
\end{align}
%
Note that this extension does not result in computational overhead at inference stage yet improves the performance even further.


\begin{figure}
	\begin{center}
        \includegraphics[width=0.95\linewidth]{figures/rtm_2.png}
        \vspace{-5mm}
	\end{center}
	\caption{Compatible training with learnable new embedding.
	Compared to Figure~\ref{fig:rtm}, another transformation module $\rho(\cdot)$ is incorporated on top of the new model to learn new embedding favorable to our rank merging. 
	The retrieval results are now merged from $\{ \rho^\text{rev}, \phi^\text{old} \}$ and $\{ \rho^\text{new}, \rho^\text{new} \}$.
	}
	\label{fig:rtm_trainable}
	\vspace{-1mm}    
\end{figure}





==> sections/Method_reverse_module.tex <==
% !TEX root = ./../main.tex


\clearpage
\section{[See Ch.6] Reverse Query Transform}
\label{sec:rtm}

Our baseline image retrieval method is model-agnostic, free from extra training, and effective for performance improvement.
However, one may argue that the proposed approach is computationally expensive at inference time because we need to conduct feature extraction twice per query for both the old and new models.
This section discusses how to alleviate this limitation by introducing a small network, called the reverse query transform module.

% \begin{figure}
% 	\begin{center}
%         \includegraphics[width=0.9\linewidth]{figures/rtm_basic.png}
%         \vspace{-0.4cm}
% 	\end{center}
% 	\caption{Reverse transformation module, $\psi_\text{rev}(\cdot)$, learns a mapping from new to old feature spaces.}
% 	\label{fig:rtm}
% 	\vspace{-0.1cm}    
% \end{figure}

\begin{figure}
	\begin{center}
        \includegraphics[width=0.9\linewidth]{figures/rtm_1.png}
        \vspace{-3mm}
	\end{center}
	\caption{Reverse query transform module, $\psi(\cdot)$, learns a mapping from new to old feature spaces.
	We only update the parameters of the module $\psi(\cdot)$ (in red rectangle) during training.
	}
	\label{fig:rtm}
	\vspace{-2mm}    
\end{figure}

\subsection{Basic Formulation}
\label{sub:formulation}

\begin{figure*}
	\begin{center}
        \includegraphics[width=0.97\linewidth]{figures/backward_system2.png}
        \vspace{-5mm}
	\end{center}
	\caption{
%	Image retrieval merging with reverse query transform module.
Image retrieval with our full rank merge framework.
%	Backward retrieval system consists of reversely transformed new query and old gallery, $\{ \phi^\text{rev}, \phi^\text{old} \}$.
%	The final image retrieval results are given by merging the outputs from $\{ \phi^\text{rev}, \phi^\text{old} \}$ and $\{ \phi^\text{new}, \phi^\text{new} \}$.
Backward retrieval system consists of reversely transformed new query and old gallery, $\{ \rho^\text{rev}, \phi^\text{old} \}$.
	The final image retrieval results are given by merging the outputs from $\{ \rho^\text{rev}, \phi^\text{old} \}$ and $\{ \rho^\text{new}, \rho^\text{new} \}$.
	}
	\label{fig:ensemble_rtm}
	\vspace{-1mm}    
\end{figure*}


To reduce the computational cost incurred by computing query embeddings twice at the inference stage, we compute the embedding using the new model and transform it to the version compatible with the old model through the reverse query transform module as illustrated in Figure~\ref{fig:rtm}.
To establish such a mechanism, we fix the parameters of the old and new models $\{ \phi^\text{old}, \phi^\text{new} \}$ after training them independently, and train a lightweight network, $\psi (\cdot)$, which transforms the embedding in the new model to the one in the old model. 
For each training example $\mathbf{x}$, our objective is minimizing the following loss:
\begin{align}
\mathcal{L}_\text{{RQT}}(\mathbf{x}) := \text{dist}\left( \psi \left(\phi^\text{new}(\mathbf{x})\right), \phi^\text{old}(\mathbf{x})
\right),
\label{eq:rev_basic}
\end{align}
where dist$(\cdot, \cdot)$ is a distance metric such as $\ell_2$ or cosine distances.
\iffalse
However, we found that using only this alignment loss makes embedding easily overfit to old space and aggravates feature discriminability.
To avoid overfitting, we employ a classification loss on top of reverse-transformed new embedding as a regularizer.
The final objective is
%
\begin{align}
\min_{\psi_{\text{rev}}} \ell(x, y) &:= \text{dist}\bigg(\phi_\text{old}(x),~\psi_{\text{rev}}\Big(\phi_\text{new}(x)\Big)\bigg) \nonumber \\
&+ \lambda\cdot \text{CE}\bigg(y,~h_\text{new}\Big(\psi_{\text{rev}} \big(\phi_\text{new}(x)\big) \Big)\bigg),
\label{eq:rev}
\end{align}
%
where $y$ is the label of input image $x$, $h_\text{new}(\cdot)$ is the classification head of new model, and \text{CE}$(\cdot, \cdot)$ and $\lambda$ denote cross-entropy loss and its weight hyperparameter.
Note that we freeze the classification head of the new model, $h_\text{new}(\cdot)$, to guide the transformed embedding that satisfies the `rules' of original new embedding, which helps to preserve feature discriminability.
\fi
Because we only update the parameters in $\psi(\cdot)$, not the ones in $\phi^\text{new}(\cdot)$ or $\phi^\text{old}(\cdot)$, we can still access the representations given by the new model at no cost even after the optimization of $\psi(\cdot)$.
%
Note that this reverse query transform module differs from FCT~\cite{fct} mainly in terms of transformation direction and requirement of side information. FCT performs a transformation from the old representation to the new, while the opposite is true for our proposed approach.
Since the embedding quality of a new model is highly likely to be better than that of an old one, our reverse transformation module performs well even without additional side information and, consequently, is more practical and efficient.

\subsection{Integration into Baseline Retrieval System}



Figure~\ref{fig:ensemble_rtm} illustrates the distance rank merge process together with the proposed reverse transformation module.
The whole procedure consists of two retrieval systems defined by a pair of query and gallery representations, backward retrieval system $\{ \phi^\text{rev}, \phi^\text{old} \}$ and new retrieval system $\{ \phi^\text{new}, \phi^\text{new} \}$, where $\phi^\text{rev} := \psi(\phi^\text{new})$.
Note that we obtain both the new and compatible query embeddings, $\phi^\text{new}(\mathbf{q})$ and $\phi^\text{rev}(\mathbf{q}) = \psi (\phi^\text{new}(\mathbf{q}))$, using a shared feature extraction network, $\phi^\text{new}(\cdot)$.

The entire image retrieval pipeline consists of two parts: 1) feature extraction of a query image and 2) search for the nearest image in a gallery from the query.
Compared to the image retrieval based on a single model, the computational cost of the proposed model with rank merge requires negligible additional cost, which corresponds to feature transformation $\psi(\cdot)$ in the first part.
{Note that the number of total gallery embeddings is fixed, \ie, $|\mathbf{G}^\text{new}|+|\mathbf{G}^\text{old}| = |\mathbf{G}|$, so the cost of the second part is always the same in both cases.}





